Improving Low-Resource Cross-lingual Parsing with Expected Statistic Regularization

We present Expected Statistic Regularization (ESR), a novel regularization technique that utilizes low-order multi-task structural statistics to shape model distributions for semi-supervised learning on low-resource datasets. We study ESR in the context of cross-lingual transfer for syntactic analysis (POS tagging and labeled dependency parsing) and present several classes of low-order statistic functions that bear on model behavior. Experimentally, we evaluate the proposed statistics with ESR for unsupervised transfer on 5 diverse target languages and show that all statistics, when estimated accurately, yield improvements to both POS and LAS, with the best statistic improving POS by +7.0 and LAS by +8.5 on average. We also present semi-supervised transfer and learning curve experiments that show ESR provides significant gains over strong cross-lingual-transfer-plus-fine-tuning baselines for modest amounts of label data. These results indicate that ESR is a promising and complementary approach to model-transfer approaches for cross-lingual parsing.

==> figs/loss-hists.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{figs/10-12_en-ewt_train_pos_freq_hists_and_losses_fig.pdf} 
    \vspace{-2em}
    \caption{\textit{Adaptive Loss Function Visualization.} Example statistic sampling distributions (sample size = 8) and their induced loss functions.  The histograms show the sampling distribution of statistics for POS tag frequency for three POS tags: {\tt PROPN}, {\tt DET}, and {\tt CCONJ}. The solid orange lines show the loss functions induced by these distributions. The samples have decreasing variance from left to right, and the respective losses adaptively become narrower in response. The vertical dotted lines show the $t_k \pm \sigma_k$ boundaries where the $\ell_k$ switches from a scaled L2 to an unscaled L1.%These plots were generated using 10,000 bootstrap batch samples from the UDv2.8-English-EWT training treebank.
    }
    \label{fig:pos-hist-loss}
\end{figure*}

==> tables/en-benchmark-results.tex <==
\begin{table*}[h!]
    \centering
    \small
    \addtolength{\tabcolsep}{-3pt}
    \begin{tabular}{lccccccccc<{\hspace{0.5cm}}c}
\toprule
& \multicolumn{10}{c}{UAS}\\
\cmidrule(lr){2-11}
{} &     zh &    fa &     ja &    id &     ko &     tr &     hi &     hr &    he &   avg \\
\midrule
\citet{He2019CrossLingualST}             &  37.26 &  \textbf{63.2} &  \textbf{43.75} &  64.2 &  37.03 &  36.05 &  33.17 &  65.31 &  64.8 &  49.4 \\
\citet{ahmad-etal-2019-cross}           &      - &     - &      - &  51.6 &  34.20 &      - &  37.40 &   63.1 &  57.2 &     - \\
\citet{Meng2019TargetLC}            &      - &     - &      - &  53.1 &  37.10 &   35.2 &  52.40 &   63.7 &  58.8 &     - \\
\citet{Kurniawan2021PPTPP}   &      - &  39.5 &      - &  50.3 &  37.50 &   39.2 &  34.00 &   63.8 &  60.5 &     - \\
\citet{Shi2021SubstructureDP}            &      - &     - &      - &     - &  \textbf{54.30} &   \textbf{56.9} &  58.30 &      - &     - &     - \\
\textsc{UDen}            &   53.5 &  54.9 &   36.1 &  67.5 &  46.70 &   53.8 &  48.80 &   82.5 &  72.8 &  57.4 \\
\textsc{UDen-PPT}        &   55.6 &  55.9 &   40.2 &  67.7 &  46.90 &   53.1 &  50.20 &   83.0 &  \textbf{77.9} &  58.9 \\
\textsc{UDen-ESR-UniArc} &   54.9 &  55.4 &   39.0 &  69.7 &  46.70 &   52.6 &  49.40 &   82.1 &  74.1 &  58.2 \\
\textsc{UDen-ESR-CLD}    &   \textbf{60.0} &  56.4 &   40.4 &  \textbf{75.6} &  50.60 &   53.1 &  \textbf{63.50} &   \textbf{83.4} &  74.1 &  \textbf{61.9} \\
\bottomrule
\end{tabular}
    \caption{\textit{UD v2.2 Unsupervised Single-Source Transfer Results.} From the comparison we see that the \textsc{UDen-ESR} approach is competitive with other state-of-the-art approaches.}
    \label{tbl:en-benchmark}
\end{table*}

==> tables/loss-agg-ablation-full-results.tex <==
\begin{table*}[t!]
    \centering
    \footnotesize
    \addtolength{\tabcolsep}{-1pt}
    \begin{tabular}{<{\hspace{0cm}}lrrrrrr<{\hspace{0.2cm}}rrrrrr<{\hspace{0.2cm}}r}
\toprule
& \multicolumn{6}{c}{POS} & \multicolumn{6}{c}{LAS} & \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
Aggregation Variant &   de &  id &  fa  &   vi &    mt &  avg &   de &    id &    fa &   vi &    mt &  avg &  avg \\
\midrule                  
Loss per sentence  & 91.2 & \textbf{86.7} & 85.1 & 67.6 & 54.7 & 77.1 & 83.8 & \textbf{64.9} & 64.4 & \textbf{49.2} & 30.4 & 58.5 & 67.8 \\
Loss per batch (ESR) & \textbf{92.6} & 86.0 & \textbf{91.0} & \textbf{68.7} & \textbf{61.0} & \textbf{79.9} &  \textbf{86.2} & 60.5 & \textbf{75.4} & 48.6 & \textbf{31.1} &  \textbf{60.4}  & \textbf{70.1}\\
\bottomrule
\end{tabular}
    \caption{\textit{Loss Aggregation Ablation Results.} } 
    \label{tbl:loss-agg-ablation-full}
\end{table*}


==> tables/loss-func-ablation-full-results.tex <==
\begin{table*}[t!]
    \centering
    \footnotesize
    \addtolength{\tabcolsep}{-1pt}
    \begin{tabular}{<{\hspace{0cm}}lrrrrrr<{\hspace{0.225cm}}rrrrrr<{\hspace{0.225cm}}r}
\toprule
& \multicolumn{6}{c}{POS} & \multicolumn{6}{c}{LAS} & \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
$\ell$ Variant &   de &  id &  fa  &   vi &    mt &  avg &   de &    id &    fa &   vi &    mt &  avg &  avg \\
\midrule                  
L2 ($\sigma=0$) & 91.5 & 87.8 & 86.2 & \textbf{70.0} & 54.7 & 78.0 & 82.9 & 64.4 & 65.0 & 48.1 & 30.4 & 58.2 & 68.1 \\
L1 ($\sigma=0$) & 91.9 & \textbf{88.1} & 87.5 & 68.7 & 56.3 & 78.5 & 85.6 & \textbf{67.1} & 67.5 & \textbf{49.9} & \textbf{32.2} & 60.3 & 69.5 \\
Hard L1 & 91.9 & \textbf{88.1} & 87.3 & 68.8 & 56.1 & 78.4 & 85.1 & 67.0 & 67.5 & 49.1 & 30.9 & 59.9 & 69.2 \\
Smooth L1 (ESR) & \textbf{92.6} & 86.0 & \textbf{91.0} & 68.7 & \textbf{61.0} & \textbf{79.9} &  \textbf{86.2} & 60.5 & \textbf{75.4} & 48.6 & 31.1 &  \textbf{60.4}  & \textbf{70.1}\\ 
\bottomrule
\end{tabular}
    \caption{\textit{Loss Function Ablation Results.} } 
    \label{tbl:loss-agg-ablation-full}
\end{table*}


==> tables/scratch-learning-curve-results.tex <==
\begin{table*}[h!]
    \definecolor{grey}{cmyk}{0.0,0.0,0.0,0.1}
    \centering
    \footnotesize
    \addtolength{\tabcolsep}{1pt}
    \begin{tabular}{lccccccccc}
    \toprule
    & \multicolumn{4}{c}{POS} & & \multicolumn{4}{c}{LAS}\\
    \cmidrule(lr){2-5} \cmidrule(lr){7-10}
    Method\hspace{60pt}$|\D^{\text{train}}_L|$ & 50 & 100 & 500 & 1000 & & 50 & 100 & 500 & 1000\\[0.1cm]
    \midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{German (de)}\\
\textsc{UDpre} & 89.6 & 89.6 & 89.6 & 89.6 & & 83.0 & 83.0 & 83.0 & 83.0 \\
\textsc{mBERT-FT} & 87.9 & \textbf{90.9} & 95.1 & \textbf{96.2} & & 59.7 & 66.7 & 81.5 & \textbf{86.3} \\
\textsc{mBERT-FT-PPT} & 86.3 & 89.6 & 94.7 & 96.0 & & 58.0 & 65.3 & 80.9 & 85.8 \\
\textsc{mBERT-FT-ESR-UniArc} & 88.1 & 90.6 & \textbf{95.2} & 96.1 & & 60.6 & 66.4 & 82.6 & 85.6 \\
\textsc{mBERT-FT-ESR-Combo} & 86.1 & 88.8 & 94.7 & 95.5 & & 57.0 & 65.0 & 82.0 & 85.6 \\
\textsc{mBERT-FT-ESR-CLD} & \textbf{88.9} & \textbf{90.9} & \textbf{95.2} & 95.8 & & \textbf{62.4} & \textbf{67.1} & \textbf{82.9} & 85.0 \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{Indonesian (id)}\\
\textsc{UDpre} & 82.3 & 82.3 & 82.3 & 82.3 & & 58.3 & 58.3 & 58.3 & 58.3 \\
\textsc{mBERT-FT} & 86.5 & 88.3 & 90.8 & 92.1 & & 52.1 & 60.6 & 71.8 & 75.2 \\
\textsc{mBERT-FT-PPT} & 86.6 & 87.9 & 90.9 & 91.8 & & 51.7 & 59.5 & 71.7 & 75.2 \\
\textsc{mBERT-FT-ESR-UniArc} & \textbf{88.4} & 89.4 & \textbf{92.2} & \textbf{93.0} & & 59.3 & 66.2 & \textbf{76.2} & \textbf{77.7} \\
\textsc{mBERT-FT-ESR-Combo} & 86.8 & 87.8 & 91.4 & 92.6 & & 58.0 & 66.2 & 74.9 & 76.0 \\
\textsc{mBERT-FT-ESR-CLD} & 88.3 & \textbf{89.9} & \textbf{92.2} & 92.9 & & \textbf{61.0} & \textbf{67.9} & 75.7 & 77.4 \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{Persian (fa)}\\
\textsc{UDpre} & 79.1 & 79.1 & 79.1 & 79.1 & & 48.4 & 48.4 & 48.4 & 48.4 \\
\textsc{mBERT-FT} & 81.1 & 83.7 & 89.6 & 91.6 & & 44.1 & 52.7 & 68.7 & 74.3 \\
\textsc{mBERT-FT-PPT} & 78.6 & 83.0 & 89.5 & 91.5 & & 35.6 & 50.7 & 68.5 & 73.6 \\
\textsc{mBERT-FT-ESR-UniArc} & 82.4 & 85.0 & 90.6 & 91.9 & & 45.2 & 57.4 & 71.6 & 74.7 \\
\textsc{mBERT-FT-ESR-Combo} & 77.9 & 82.8 & 90.1 & 91.7 & & 36.4 & 51.9 & 70.3 & 74.7 \\
\textsc{mBERT-FT-ESR-CLD} & \textbf{82.8} & \textbf{85.8} & \textbf{90.7} & \textbf{92.1} & & \textbf{50.3} & \textbf{59.5} & \textbf{71.8} & \textbf{75.0} \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{Vietnamese (vi)}\\
\textsc{UDpre} & 67.0 & 67.0 & 67.0 & 67.0 & & 46.3 & 46.3 & 46.3 & 46.3 \\
\textsc{mBERT-FT} & 79.7 & 81.7 & 86.8 & 88.4 & & 31.6 & 39.9 & 53.9 & 57.2 \\
\textsc{mBERT-FT-PPT} & 78.3 & 81.6 & 86.9 & 88.6 & & 31.1 & 39.1 & 54.2 & 57.0 \\
\textsc{mBERT-FT-ESR-UniArc} & 83.1 & \textbf{85.7} & \textbf{88.1} & 88.8 & & 44.3 & 50.3 & 56.4 & \textbf{57.9} \\
\textsc{mBERT-FT-ESR-Combo} & 80.7 & 84.2 & 87.9 & \textbf{88.9} & & 43.8 & 49.2 & \textbf{56.7} & 57.4 \\
\textsc{mBERT-FT-ESR-CLD} & \textbf{83.6} & 85.6 & 88.0 & 88.7 & & \textbf{44.7} & \textbf{50.8} & 56.6 & \textbf{57.9} \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{Maltese (mt)}\\
\textsc{UDpre} & 35.1 & 35.1 & 35.1 & 35.1 & & 16.0 & 16.0 & 16.0 & 16.0 \\
\textsc{mBERT-FT} & 74.3 & 78.8 & 88.2 & 90.5 & & 35.0 & 41.5 & 59.0 & 64.0 \\
\textsc{mBERT-FT-PPT} & 74.3 & 78.9 & 88.1 & 90.6 & & 35.4 & 41.7 & 58.7 & 63.7 \\
\textsc{mBERT-FT-ESR-UniArc} & 82.2 & \textbf{86.4} & \textbf{90.3} & 91.5 & & 47.0 & 54.4 & 64.2 & 67.3 \\
\textsc{mBERT-FT-ESR-Combo} & 80.2 & 85.6 & \textbf{90.3} & \textbf{91.6} & & 43.4 & 53.7 & 63.7 & \textbf{67.7} \\
\textsc{mBERT-FT-ESR-CLD} & \textbf{82.3} & 86.2 & \textbf{90.3} & 91.5 & & \textbf{47.5} & \textbf{54.7} & \textbf{64.3} & 67.2 \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{All (avg)}\\
\textsc{UDpre} & 70.6 & 70.6 & 70.6 & 70.6 & & 50.4 & 50.4 & 50.4 & 50.4 \\
\textsc{mBERT-FT} & 81.9 & 84.7 & 90.1 & 91.8 & & 44.5 & 52.3 & 67.0 & 71.4 \\
\textsc{mBERT-FT-PPT} & 80.8 & 84.2 & 90.0 & 91.7 & & 42.4 & 51.3 & 66.8 & 71.0 \\
\textsc{mBERT-FT-ESR-UniArc} & 84.8 & 87.4 & \textbf{91.3} & \textbf{92.3} & & 51.3 & 58.9 & \textbf{70.2} & \textbf{72.6} \\
\textsc{mBERT-FT-ESR-Combo} & 82.3 & 85.8 & 90.9 & 92.1 & & 47.7 & 57.2 & 69.5 & 72.3 \\
\textsc{mBERT-FT-ESR-CLD} & \textbf{85.2} & \textbf{87.7} & \textbf{91.3} & 92.2 & & \textbf{53.2} & \textbf{60.0} & \textbf{70.2} & 72.5 \\
    \bottomrule
    \end{tabular} 
    \caption{\textit{\textsc{mBERT} Semi-Supervised Learning Curves.}}
\end{table*}


==> tables/ud-13-learning-curve-results.tex <==
\begin{table*}[h!]
    \definecolor{grey}{cmyk}{0.0,0.0,0.0,0.1}
    \centering
    \footnotesize
    \addtolength{\tabcolsep}{1pt}
    \begin{tabular}{lccccccccc}
    \toprule
    & \multicolumn{4}{c}{POS} & & \multicolumn{4}{c}{LAS}\\
    \cmidrule(lr){2-5} \cmidrule(lr){7-10}
    Method\hspace{60pt}$|\D^{\text{train}}_L|$ & 50 & 100 & 500 & 1000 & & 50 & 100 & 500 & 1000\\[0.1cm]
    \midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{German (de)}\\
\textsc{UDpre} & 89.6 & 89.6 & 89.6 & 89.6 & & 83.0 & 83.0 & 83.0 & 83.0 \\
\textsc{UDpre-FT} & \textbf{94.4} & \textbf{95.8} & 96.9 & \textbf{97.2} & & 87.9 & 89.3 & \textbf{91.6} & \textbf{92.3} \\
\textsc{UDpre-FT-PPT} & 94.1 & 95.4 & 96.7 & 97.1 & & \textbf{88.3} & \textbf{89.4} & 91.4 & \textbf{92.3} \\
\textsc{UDpre-FT-ESR-UniArc} & 94.2 & 95.6 & \textbf{96.9} & \textbf{97.2} & & 87.4 & 89.0 & 91.3 & \textbf{92.3} \\
\textsc{UDpre-FT-ESR-Combo} & 93.8 & 95.0 & 96.4 & 96.9 & & 87.3 & 88.7 & 91.0 & 92.0 \\
\textsc{UDpre-FT-ESR-CLD} & 94.1 & 95.0 & 96.7 & \textbf{97.2} & & 87.4 & 88.9 & 91.1 & 92.2 \\
\textsc{UDpre-FT-ESR-CLD$^*$} & 94.2 & 95.2 & 96.7 & \textbf{97.2} & & 87.5 & 88.8 & 91.1 & 92.1 \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{Indonesian (id)}\\
\textsc{UDpre} & 82.3 & 82.3 & 82.3 & 82.3 & & 58.3 & 58.3 & 58.3 & 58.3 \\
\textsc{UDpre-FT} & 89.7 & 90.0 & 92.0 & 92.2 & & 71.8 & 74.4 & 77.5 & 78.5 \\
\textsc{UDpre-FT-PPT} & 89.9 & 90.2 & 92.3 & 92.6 & & 72.4 & 74.7 & 78.0 & 79.1 \\
\textsc{UDpre-FT-ESR-UniArc} & \textbf{91.3} & \textbf{91.9} & 92.9 & \textbf{93.1} & & \textbf{75.4} & 76.4 & \textbf{79.3} & \textbf{80.0} \\
\textsc{UDpre-FT-ESR-Combo} & 89.4 & 89.6 & 92.6 & 92.9 & & 72.4 & 75.0 & 78.8 & \textbf{80.0} \\
\textsc{UDpre-FT-ESR-CLD} & 90.7 & 91.6 & 92.8 & \textbf{93.1} & & 74.6 & 76.5 & 79.1 & \textbf{80.0} \\
\textsc{UDpre-FT-ESR-CLD$^*$} & 90.6 & 91.8 & \textbf{93.0} & 93.0 & & 73.8 & \textbf{76.8} & 79.1 & 79.9 \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{Persian (fa)}\\
\textsc{UDpre} & 79.1 & 79.1 & 79.1 & 79.1 & & 48.4 & 48.4 & 48.4 & 48.4 \\
\textsc{UDpre-FT} & 90.9 & 91.7 & 93.7 & 94.2 & & \textbf{74.9} & \textbf{77.0} & 80.9 & 83.0 \\
\textsc{UDpre-FT-PPT} & 90.5 & \textbf{91.8} & \textbf{93.9} & 94.2 & & 74.7 & 76.9 & \textbf{81.0} & 82.7 \\
\textsc{UDpre-FT-ESR-UniArc} & 90.9 & 91.1 & 93.5 & \textbf{94.5} & & 73.0 & 75.6 & 80.6 & 83.1 \\
\textsc{UDpre-FT-ESR-Combo} & 90.1 & 91.3 & 93.4 & 94.3 & & 74.2 & 76.3 & 80.8 & \textbf{83.5} \\
\textsc{UDpre-FT-ESR-CLD} & 90.5 & 91.3 & 93.5 & 94.3 & & 72.9 & 75.3 & 80.8 & 82.5 \\
\textsc{UDpre-FT-ESR-CLD$^*$} & \textbf{91.1} & 91.1 & 93.5 & \textbf{94.5} & & 74.3 & 75.9 & 80.8 & 83.2 \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{Vietnamese (vi)}\\
\textsc{UDpre} & 67.0 & 67.0 & 67.0 & 67.0 & & 46.3 & 46.3 & 46.3 & 46.3 \\
\textsc{UDpre-FT} & 86.3 & 87.1 & 90.0 & 91.5 & & 55.8 & 56.9 & 63.7 & 65.9 \\
\textsc{UDpre-FT-PPT} & 86.3 & 87.3 & 90.2 & \textbf{91.6} & & 57.1 & 57.7 & 64.0 & \textbf{66.5} \\
\textsc{UDpre-FT-ESR-UniArc} & \textbf{87.9} & 88.7 & 91.3 & 91.4 & & \textbf{58.8} & 60.6 & \textbf{65.4} & 65.7 \\
\textsc{UDpre-FT-ESR-Combo} & 86.3 & 88.2 & 91.0 & 91.3 & & 58.2 & 59.7 & 65.1 & 66.3 \\
\textsc{UDpre-FT-ESR-CLD} & 87.0 & 88.7 & \textbf{91.4} & 91.5 & & 58.3 & 60.4 & 65.3 & 65.8 \\
\textsc{UDpre-FT-ESR-CLD$^*$} & 87.0 & \textbf{90.5} & \textbf{91.4} & 91.4 & & 58.5 & \textbf{64.5} & 65.3 & 65.6 \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{Maltese (mt)}\\
\textsc{UDpre} & 35.1 & 35.1 & 35.1 & 35.1 & & 16.0 & 16.0 & 16.0 & 16.0 \\
\textsc{UDpre-FT} & 82.9 & 86.4 & 92.9 & 94.3 & & 57.9 & 64.5 & 75.7 & 79.4 \\
\textsc{UDpre-FT-PPT} & 83.8 & 87.6 & 93.2 & 94.3 & & 59.3 & 65.6 & 76.1 & 80.0 \\
\textsc{UDpre-FT-ESR-UniArc} & \textbf{92.2} & 91.7 & \textbf{93.7} & \textbf{94.5} & & \textbf{75.1} & 73.3 & 78.0 & 79.9 \\
\textsc{UDpre-FT-ESR-Combo} & 88.0 & 92.1 & 93.6 & 94.4 & & 73.4 & 75.9 & \textbf{78.3} & \textbf{80.1} \\
\textsc{UDpre-FT-ESR-CLD} & 91.4 & \textbf{93.2} & 93.4 & \textbf{94.5} & & 73.4 & \textbf{76.6} & 78.1 & 80.0 \\
\textsc{UDpre-FT-ESR-CLD$^*$} & 89.7 & 91.7 & 93.5 & 94.4 & & 69.7 & 74.3 & 78.2 & 79.8 \\
\midrule
    \rowcolor{grey}
    \multicolumn{10}{c}{All (avg)}\\
\textsc{UDpre} & 70.6 & 70.6 & 70.6 & 70.6 & & 50.4 & 50.4 & 50.4 & 50.4 \\
\textsc{UDpre-FT} & 88.8 & 90.2 & 93.1 & 93.9 & & 69.7 & 72.4 & 77.9 & 79.8 \\
\textsc{UDpre-FT-PPT} & 88.9 & 90.5 & 93.3 & 94.0 & & 70.4 & 72.9 & 78.1 & 80.1 \\
\textsc{UDpre-FT-ESR-UniArc} & \textbf{91.3} & 91.8 & \textbf{93.7} & \textbf{94.1} & & \textbf{73.9} & 75.0 & \textbf{78.9} & 80.2 \\
\textsc{UDpre-FT-ESR-Combo} & 89.5 & 91.3 & 93.4 & 94.0 & & 73.1 & 75.1 & 78.8 & \textbf{80.4} \\
\textsc{UDpre-FT-ESR-CLD} & 90.8 & 92.0 & 93.6 & \textbf{94.1} & & 73.3 & 75.6 & \textbf{78.9} & 80.1 \\
\textsc{UDpre-FT-ESR-CLD$^*$} & 90.5 & \textbf{92.1} & 93.6 & \textbf{94.1} & & 72.8 & \textbf{76.0} & \textbf{78.9} & 80.1 \\
    \bottomrule
    \end{tabular} 
    \caption{\textit{\textsc{UDpre} Semi-Supervised Learning Curves.}}
\end{table*}

